An Execution Model for RICE

In this paper, we build on the previous work of the RICE compiler by giving its execution model. We show the restrictions to the FlatCurry language that were made to produce executable code, and present the execution model using operational semantics similar to Launchbury. Finally, we show that the execution model conforms with the standard operational semantics for Curry.

==> eptcsdata.tex <==
\providecommand{\firstpage}{112}
\providecommand{\publicationstatus}{Cynthia Kop and Helida Salles Santos (Eds); 19th Workshop on\\ Logical and Semantic Frameworks with Applications (LSFA'24)\\
EPTCS 421, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.421.7}{10.4204/EPTCS.421.7}}

